MeshMask: Physics-Based Simulations with Masked Graph Neural Networks

We introduce a novel masked pre-training technique for graph neural networks (GNNs) applied to computational fluid dynamics (CFD) problems. By randomly masking up to 40\% of input mesh nodes during pre-training, we force the model to learn robust representations of complex fluid dynamics. We pair this masking strategy with an asymmetric encoder-decoder architecture and gated multi-layer perceptrons to further enhance performance. The proposed method achieves state-of-the-art results on seven CFD datasets, including a new challenging dataset of 3D intracranial aneurysm simulations with over 250,000 nodes per mesh. Moreover, it significantly improves model performance and training efficiency across such diverse range of fluid simulation tasks. We demonstrate improvements of up to 60\% in long-term prediction accuracy compared to previous best models, while maintaining similar computational costs. Notably, our approach enables effective pre-training on multiple datasets simultaneously, significantly reducing the time and data required to achieve high performance on new tasks. Through extensive ablation studies, we provide insights into the optimal masking ratio, architectural choices, and training strategies.

==> background.tex <==
The success of Convolutional Neural Networks (CNN) in image processing \cite{imagenet, alexnet} prompted their direct application to Computational Fluid Dynamics (CFD). One significant application involves mapping meshes or velocity and pressure fields into images to exploit such CNNs. \cite{Tompson2016} conducted 3D-fluid simulations employing a CNN that forecasts subsequent images based on preceding ones. Similarly, both \cite{Thuerey2018} and \cite{Chen2019} utilized a U-net architecture to predict pressure and velocity fields given solely a shape as input. However, these approaches were not applied to sequences of meshes/images and cannot leverage the power of unstructured grids.

Concurrently, \cite{Battaglia2016} and \cite{sanchezgonzalez2020learning} constructed a framework based on Graph Neural Networks (GNNs) that made it possible to process unstructured grids or meshes directly. \cite{pfaff2021learning} achieved state-of-the-art results with such an approach, albeit restricted to small meshes (under 4000 nodes). To overcome this limitation, \cite{Yang2022amgnet, taghibakhshi2023mggnn,lino2021simulating} employ multiple graph coarsening stages, while \cite{Fortunato2022} builds and operates with two graphs of different refinement stages from the start. Returning to CNNs, this MultiGrid approach can be put in parallel with U-net architectures \cite{ronneberger2015unet,lin2017feature}. In its simplest form, devoid of skip-connections, a U-net can be likened to a basic multigrid V-cycle for images. With the incorporation of skip-connections, a more intricate W-cycle emerges.

Beginning with Natural Language Processing (NLP), Transformers \cite{vaswani2023attention} achieved state-of-the-art results by replacing CNN and Recurrent layers with Self-Attention and Multi-Layer Perceptron (MLP). They now achieve state-of-the-art results in Computer Vision and Image Generation \cite{dosovitskiy2021image, arnab2021vivit} as well. While Transformers were introduced for GNNs before\cite{yun2020graph,müller2023attending,veličković2018graph}, those operations were primarily created for spatial fashion and not for sequences of graphs. \cite{shi2021masked} introduce a Self-Attention mechanism to coarsen a graph, bridging the gap with the MultiGrid approaches seen above.

\cite{devlin2019bert} constructed a framework where tokens from a sentence are being masked before being passed to a model. This method is now a key element of any LLM training. \cite{he2021masked} adapts the same approach for images, while masking a much larger amounts of information (up to 85\% of an image). \cite{Hu2019} masked a fraction of the nodes' features, but keep the structural integrity of the graphs they work with. \cite{Tan2022} masked some subset of edges before reconstructing the final graph with an Auto Encoder architecture, similar to \cite{he2021masked}.

In this paper, we develop a dynamic MultiGrid approach to spatially process meshes. Our architecture can autoregressively predict full CFD simulations from a minimal amount of inputs. We also present a novel pre-training task for Graph that leads in a boost of performance.
